RTMPose: Real-Time Multi-Person Pose Estimation based on MMPose

Recent studies on 2D pose estimation have achieved excellent performance on public benchmarks, yet its application in the industrial community still suffers from heavy model parameters and high latency. In order to bridge this gap, we empirically explore key factors in pose estimation including paradigm, model architecture, training strategy, and deployment, and present a high-performance real-time multi-person pose estimation framework, RTMPose, based on MMPose. Our RTMPose-m achieves 75.8% AP on COCO with 90+ FPS on an Intel i7-11700 CPU and 430+ FPS on an NVIDIA GTX 1660 Ti GPU, and RTMPose-l achieves 67.0% AP on COCO-WholeBody with 130+ FPS. To further evaluate RTMPose's capability in critical real-time applications, we also report the performance after deploying on the mobile device. Our RTMPose-s achieves 72.2% AP on COCO with 70+ FPS on a Snapdragon 865 chip, outperforming existing open-source libraries. Code and models are released at https://github.com/open-mmlab/mmpose/tree/1.x/projects/rtmpose.

==> sections/bak/methods_bak.tex <==
% !TEX root = ../main.tex

\section{Methodology}

In this work, we adopt the SimCC~\cite{SimCC} method with CSPNeXt-m as the backbone and remove the transposed convolutional layers in the standard implementation. We use a large kernel convolutional layer and a fully-connected layer to improve the model performance.  We also use an efficient self-attention module to model the intrinsic structural constraints. In addition, we adopt the training strategy proposed in \cite{lyu2022rtmdet} with slight modifications, and show it generally improves the performance of pose estimation models. The final model architecture is shown in Fig.~\ref{fig:model}. We also illustrate the roadmap of step-by-step improvements in Fig.~\ref{fig:roadmap}.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.46\textwidth]{./figs/model.pdf}
%     % \vspace{-.8em}
%     \caption{Model Architecture}
%     \label{fig:model}
%     % \vspace{-1.5em}
% \end{figure}


% \begin{figure}[htbp]
%     % \centering
%     \includegraphics[width=0.5\textwidth]{./figs/roadmap.pdf}
%     % \vspace{-.8em}
%     \caption{Step-by-step improvements from a SimCC baseline model.}
%     \label{fig:roadmap}
%     % \vspace{-1.5em}
% \end{figure}

\subsection{Preliminary: SimCC}

SimCC~\cite{SimCC} is a new method that does not belong to heatmap-based~\cite{xiao2018simple, huang2020devil, Zhang_2020_CVPR, xu2022vitpose} and regression-based methods~\cite{Toshev_2014_CVPR, li2021human, mao2022poseur}, it has a very simple structure, using one $1\times1$ convolution layer to transform features extracted by backbone to keypoint representations, and two fully-connected layers to perform classification respectively. 

The core idea of SimCC is to divide the horizontal and vertical axes uniformly into multiple consecutively numbered bins, and to treat the integer index of each bin as a class label during model training. By dividing a larger number of bins than the aspect of the input image, the quantization error can be reduced to sub-pixel level.

In addition to the standard one-hot form, inspired by label smoothing in traditional classification tasks, SimCC also proposes a Gaussian label smoothing to smooth the training label following the Gaussian distribution. This technique introduces an inductive bias in the soft labels to give higher weights to pixels that are close to the groundtruth, thus greatly improving the model performance. We find that this technique is very similar to the idea of the SORD~\cite{sord} algorithm in ordinal regression task. These soft labels naturally encapsulate the rank likelihoods of an input instance given a pre-defined interclass penalty distance.

\subsection{A lightweight but strong baseline}

\paragraph{SimCC without upsampling layers}
We compare SimCC and the heatmap-based method proposed in \cite{xiao2018simple} using ResNet-50~\cite{he2016deep} as the backbone.  As shown in Table~\ref{tab:ablation:rm_upsampling}, with the removal of upsampling layers, SimCC can still achieve similar localization accuracy as the heatmap-based method~\cite{xiao2018simple}. We believe that this approach of encoding global spatial information into one dimension is more efficient for localization tasks. When replacing the backbone of this simple yet but strong baseline model with CSPNeXt-m and training it from scratch, we achieve 69.7\% AP. 

%tab:ablation_rm_upsampling
\begin{table}[htb]
\centering
\caption{Computational costs and accuracy of different methods. For comparison purposes, we only show FLOPs and model parameters of prediction heads. ``SimCC*'' denotes the removal of upsampling layers from standard SimCC head.}\label{tab:ablation:rm_upsampling}
\vspace{3pt}
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{ccccc}
\hline
Method  & Feature Size & FLOPs(G) & Params(M) & AP  \\ \hline
Heatmap & 64x48 & 1.426         & 10.492         & 71.8 \\
SimCC*   & 512+384   & 0.002         & 0.079          & 71.3 \\ \hline
\end{tabular}}
\end{table}

% We compare SimCC and the heatmap-based method proposed in \cite{xiao2018simple}. In the standard SimCC implementation, it only adds two fully-connected layers to the heatmap-based approach, which changes the supervised signal from a two-dimensional Gaussian heatmap to a one-dimensional Gaussian distribution.

% In the heatmap-based method, the final prediction is obtained by $1\times1$ convolution, which is totally equivalent to a position-wise linear transformation layer, essentially computing the inner product of the $1\times1$ convolution kernel and each pixel token, i.e., computing the vector similarity. Thus the model optimizes the quality of representation of each pixel token, and what is learned is the local pixel representation of each keypoint. 

% As for SimCC, each vector is transformed from a 2-d feature map, so it contains global spatial information. When classifying this vector with the fully connected layer, it essentially calculates the similarity of this vector to each coordinate representation, and the positional representation is learned.  
% Therefore, for heatmap-based methods, the number of pixels must be increased by upsampling layers to reduce the quantization error, while the positional representation only needs to learn discriminative features, which enables the required feature dimension to be low. As shown in Table 1, with the removal of upsampling layers, 48-dimensional vectors SimCC use can still achieve similar localization accuracy as the 64x48, i.e., 2000+ dimensional representation in \cite{xiao2018simple}. We believe that this architecture of encoding global spatial information in one dimension is more efficient for localization tasks.

% \paragraph{Removing the classification backbone's last convolutional layer}
% Many of the backbones we currently use are designed for image classification tasks, and there are some conventions implicit in them that are only valid for classification tasks. For example, models such as [pplcnet] will use a high-dimensional 1x1 convolution in the last layer of the backbone to raise the feature dimension. In practice, this trick does slightly improve the model accuracy for the classification task, but for the pose estimation task it does not bring a significant improvement but adds a lot of computation.

\subsection{Training Techniques}\label{sec:training_techniques}

\paragraph{Pre-training}

It has been shown in works such as \cite{blazepose, li2021human} that pre-training the backbone using the heatmap-based method can improve the model accuracy. We adopt UDP~\cite{Huang_2020_CVPR} method for the backbone pre-training. This improves the model from 69.7\% AP to 70.3\% AP. From now on, we will use this technique by default.

\paragraph{Optimization Strategy}

We refer to the optimization strategy used in \cite{lyu2022rtmdet}. The Exponential Moving Average (EMA) is used for alleviating the overfitting (70.3\% to 70.4\%). The Flat Cosine Annealing strategy improves the accuracy to 70.7\% AP. We also inhibit weight decay on normalization layers and biases. 

%Experiments show that using Adam on the baseline model achieves better results (71.2\%) than using AdamW\cite{ADAMW} with a weight decay of 0.05 (69.9\%), but with the addition of modules, the risk of overfitting the model becomes greater, when using AdamW yields better performance.

\paragraph{Two-stage training augmentations}

We follow the training strategy from \cite{lyu2022rtmdet}, adopt a strong and weak two-stage augmentation. First using stronger data augmentations to train 180 epochs and then a weaker strategy for 30 epochs. During the strong stage, we use a larger random scaling range [0.6, 1.4], and a larger random rotation factor, 80, and set the CoarseDropout probability to 1. According to AID~\cite{aid}, CoarseDropout helps to alleviate the model's overfitting to the image texture information and encourages it to learn the pose structure information. In the weak strategy stage, we turn off the random shift, use a smaller random rotation range, and set the CoarseDropout probability to 0.5 to allow the model to fine-tune in a domain that more closely matches the real image feature distribution. Experiments show that using Adam on the baseline model achieves a better result (71.2\% AP) than using AdamW~\cite{ADAMW} with a weight decay of 0.05 (69.9\% AP). However, in later experiments we found that with the addition of more modules, AdamW could achieve better performance.
\begin{figure}[tbp]
    % \centering
    \includegraphics[width=0.5\textwidth]{./figs/roadmap3.pdf}
    % \vspace{-.8em}
    \caption{Step-by-step improvements from a SimCC baseline.}
    \label{fig:roadmap}
    % \vspace{-1.5em}
\end{figure}
\subsection{Module Design}

\paragraph{Feature dimension}

Since it is observed that the model performance increases when the feature map is at higher resolution, we use a fully connected layer to up-dimension the 1D vector, and the feature dimension can be adjusted as a hyper-parameter. In this work, we use 256 dimensions and the accuracy is changed from 71.2\% AP to 71.4\% AP.

\paragraph{Self-attention module}

An efficient Transformer variant, Gated Attention Unit(GAU), was proposed in \cite{Hua2022TransformerQI}, which still has a quadratic complexity, but has faster speed, lower memory cost, and better results than the vanilla Transformer.
\begin{figure*}[htbp]
    % \centering
    \includegraphics[width=\textwidth]{./figs/pipeline2.pdf}
    % \vspace{-.8em}
    \caption{Inference pipeline of RTMPose.}
    \label{fig:pipeline}
    % \vspace{-1.5em}
\end{figure*}
In the standard Transformer layer, feed-forward networks(FFN) and attention layers are used in pairs, with a multi-head self-attention module to improve feature diversity. But it was found that the Gated Linear Unit(GLU)~\cite{glu} form of FFN works better:
\begin{equation}
    O=(U\odot V)W_o, U=\phi_u(XW_{u}), V=\phi_v(XW_{v})
\end{equation}
where $\odot$ is the pairwise multiplication (Hadamard product) and $\phi$ is the activation function. GAU improves on the GLU by integrating attention mechanism in an elegant form:
\begin{equation}
O=(U \odot AV)W_o
\end{equation}
Our implementation is as follows:
\begin{equation}
A = \frac {1}{n} \mathit{relu} ^2( \frac {Q(X)K(Z)^\top}{ \sqrt {s} }), Z=\phi_z( X W_z)
\end{equation}
where $s = 128$, $Q$ and $K$ are simple linear transformations, and $\mathit{relu}^2(\cdot )$ is ReLU then squared. Since work such as \cite{li2021tokenpose, yang2021transpose} demonstrated that the attention mechanism is beneficial for structural information learning in pose estimation tasks, we added GAU to improve the robustness to occlusion and verified the effectiveness experimentally. This self-attention module brings the model by 0.5\% AP (71.9\%) improvement.

\subsection{Micro Design}

\paragraph{Loss function}

A soft label encoding paradigm is proposed in SORD~\cite{sord}:
\begin{equation}
y_i=\frac{e^{-\phi(r_t, r_i)}}{\sum^K_{k=1}e^{-\phi(r_t,r_k)}}
\end{equation}
where $\phi(r_t, r_i)$ is a metric loss function of our choice that penalizes how far the true metric value of $r_t$ is from the rank $r_i \in Y$, and this formula can be seen as computing Softmax for all $-\phi(r_t, r_i)$. In this work, we adopt the unnormalized Gaussian distribution as the inter-class distance metric:
\begin{equation}
\phi(r_t, r_i)=e^{\frac{-(r_t-r_i)^2}{2\sigma^2}}
\end{equation}
A Softmax with temperature was used for both the model output and the soft labels.
\begin{equation}
y_i=\frac{e^{-\phi(r_t, r_i)/\tau}}{\sum^L_{l=1}e^{-\phi(r_t,r_l)/\tau}}
\end{equation}
to further adjust the normalized distribution shape. According to the experimental results, taking $\tau=1/10$ can improve the performance from 71.9\% to 72.7\%. 

\paragraph{Separate $\sigma$}
In SimCC, the horizontal and vertical soft labels are encoded using the same $\sigma$, and we empirically explore a simple strategy to set separate $\sigma$ for them.
\begin{equation}
\sigma = \sqrt{\frac{W_{S}}{16}}
\end{equation}
where $W_{S}$ is the length of the SimCC vector. This step changes the accuracy from 72.7\% to 72.8\%.

\paragraph{Final convolutional layer}

We experiment with different kernel sizes of convolutional kernels for feature fusion, and we find that using a larger kernel size gives a performance improvement over using $1\times1$ convolution, and finally we chose $7\times7$ convolution as the last convolutional layer, which achieves 73.3\% AP. We compare model performances of different kernel sizes as shown in Table~\ref{tab:ablation:kernel_sizes}. Additionally, we also conduct experiments on the final model for the effect of different temperature factors and the results are shown in Table.~\ref{tab:ablation:temperature}

% \begin{table}[htbp]
% \centering
% \caption{Comparison of different kernel sizes}\label{tab:ablation:kernel_sizes}
% \vspace{3pt}
% \begin{tabular}{ll}
% \hline
% Kernel Size & mAP  \\ \hline
% 1x1         & 72.8 \\
% 3x3         & 73.2 \\
% 5x5         & 73.2 \\
% \ours{7x7}  & \ours{73.3} \\
% 9x9         & 73.0 \\
% \hline
% \end{tabular}
% \end{table}

% \begin{table}[htbp]
% \centering
% \caption{Comparison of different temperature factors.}\label{tab:ablation:temperature}
% \vspace{3pt}
% \begin{tabular}{cc}
% \hline
% $\tau$ & mAP  \\ \hline
% 1         & unstable \\
% 5         & 73.1 \\
% \ours{10} & \ours{73.3} \\
% 15         & 73.0 \\
% \hline
% \end{tabular}
% \end{table}
\begin{table}
    \centering
    \begin{minipage}{0.45\linewidth}
        \centering
        \caption{Comparison of different kernel sizes}\label{tab:ablation:kernel_sizes}
        \vspace{3pt}
        \begin{tabular}{ll}
        \hline
        Kernel Size & mAP  \\ \hline
        1x1         & 72.8 \\
        3x3         & 73.2 \\
        5x5         & 73.2 \\
        \ours{7x7}  & \ours{73.3} \\
        9x9         & 73.0 \\
        \hline
        \end{tabular}
    \end{minipage}
    \hfill
    \begin{minipage}{0.45\linewidth}
        \centering
        \caption{Comparison of different temperature factors.}\label{tab:ablation:temperature}
        \vspace{3pt}
        \begin{tabular}{cc}
        \hline
        $\tau$ & mAP  \\ \hline
        1         & unstable \\
        5         & 73.1 \\
        \ours{10} & \ours{73.3} \\
        15         & 73.0 \\
        \hline
        \end{tabular}
    \end{minipage}
\end{table}
% \renewcommand{\dblfloatpagefraction}{.8}
\begin{table*}[t]
	\begin{center}
 \caption{Body pose estimation results on COCO validation set. We only report GFLOPs of pose model and ignore the detection model. Flip test is not used.}
 \vspace{-3pt}
 \label{tab:compare_coco}
    \resizebox{\linewidth}{!}{
		\begin{tabular}{c|l|c|c|c|c|c|c|c}
		    \toprule
			\multicolumn{2}{c|}{Methods} 
            & Backbone & Detector & Det. Input Size & Pose Input Size & GFLOPs & AP & Extra Data  \\
			\midrule
			\multirow{6}{*}{PaddleDetection~\cite{ppdet2019}} 
   %%%%%%%%%%%%%%%
   %          & TinyPose & Wider Naive LiteHRNet & GT & - & $128 \times 96$ & 0.08 & 58.4  \\ 
			% &  TinyPose & Wider Naive LiteHRNet & GT & - & $256 \times 192$ & 0.33 & 68.3  & AIC(220K) \\ 
   %          \cmidrule{2-8}
			% & TinyPose & Wider Naive LiteHRNet & PicoDet-s & $320 \times 320$ & $128 \times 96$ & 0.08 & 52.3 &+Internal(unknown) \\ 
			% & TinyPose & Wider Naive LiteHRNet & PicoDet-s & $320 \times 320$ & $256 \times 192$ & 0.33 & 56.5  \\ 
   %%%%%%%%%%%%%%%
            & TinyPose & Wider NLiteHRNet & YOLOv3 & $608 \times 608$ & $128 \times 96$ & 0.08 & 52.3  \\ 
			& TinyPose & Wider NLiteHRNet & YOLOv3 & $608 \times 608$ & $256 \times 192$ & 0.33 & 60.9  \\ 
            \cmidrule{2-8}
            & TinyPose & Wider NLiteHRNet & Faster-RCNN & N/A & $128 \times 96$ & 0.08 & 56.1 & AIC(220K) \\ 
			& TinyPose & Wider NLiteHRNet & Faster-RCNN & N/A & $256 \times 192$ & 0.33 & 65.6 &+Internal(unknown) \\ 
            \cmidrule{2-8}
			& TinyPose & Wider NLiteHRNet & PicoDet-s & $320 \times 320$ & $128 \times 96$ & 0.08 & 48.4  \\ 
			& TinyPose & Wider NLiteHRNet & PicoDet-s & $320 \times 320$ & $256 \times 192$ & 0.33 & 56.5  \\ 
   %          \cmidrule{2-8}
   %          & TinyPose & Wider Naive LiteHRNet & RTMDet-nano & $320 \times 320$ & $128 \times 96$ & 0.08 & 40.6 \\ 
			% & TinyPose & Wider Naive LiteHRNet & RTMDet-nano & $320 \times 320$ & $256 \times 192$ & 0.33 & 47.2 \\ 
            % \midrule
   %          \multirow{2}{*}{MediaPipe} 
   %          & MoveNet-Lightning & MobileNetv2 & GT & - & $192 \times 192$ & 0.54 & 66.7  &\multirow{2}{*}{Internal(23.5K)}\\ 
			% & MoveNet-Thunder & MobileNetv2 x1.75 & GT & - & $256 \times 256$ & 2.44 & 77.9  \\ 
   %          & BlazePose-Lite & - & GT & - & $256 \times 256$ & 0.003 & 29.3  &\multirow{2}{*}{Internal(85K)}\\ 
			% & BlazePose-Full & - & GT & - & $256 \times 256$ & 0.007 & 35.4  \\ 
   % 			& BlazePose-Heavy & - & GT & - & $256 \times 256$ & 2.44 & 37.5  \\ 
            \midrule
            \multirow{6}{*}{AlphaPose~\cite{alphapose}} 
   %          & FastPose & ResNet 50 & GT & - & $256 \times 192$ & 5.91 & 73.2 &\multirow{9}{*}{-} \\ 
			% & FastPose(DUC) & ResNet-50 & GT & - & $256 \times 192$ & 9.71 & 73.5 \\ 
			% & FastPose(DUC) & ResNet-152 & GT & - & $256 \times 192$ & 15.99 & 74.8 \\ 
   %          \cmidrule{2-8}
			& FastPose & ResNet 50 & YOLOv3 & $608 \times 608$ & $256 \times 192$ & 5.91 & 71.2 &\multirow{6}{*}{-} \\ 
			& FastPose(DUC) & ResNet-50 & YOLOv3 & $608 \times 608$ & $256 \times 192$ & 9.71 & 71.7 \\ 
			& FastPose(DUC) & ResNet-152 & YOLOv3 & $608 \times 608$ & $256 \times 192$ & 15.99 & 72.6 \\ 
            \cmidrule{2-8}
            & FastPose & ResNet 50 & Faster-RCNN & N/A & $256 \times 192$ & 5.91 & 69.7 \\ 
			& FastPose(DUC) & ResNet-50 & Faster-RCNN & N/A & $256 \times 192$ & 9.71 & 70.3 \\ 
			& FastPose(DUC) & ResNet-152 & Faster-RCNN & N/A & $256 \times 192$ & 15.99 & 71.3 \\ 
			\midrule
			\multirow{22}{*}{MMPose~\cite{mmpose2020}}
            % & RTMPose-tiny & CSPNeXt-tiny & GT & - & $256 \times 192$ & 0.36 & 66.9 &\multirow{4}{*}{-}\\ 
            % & RTMPose-s & CSPNeXt-s & GT & - & $256 \times 192$ & 0.68 & 71.1 \\ 
            % & RTMPose-m & CSPNeXt-m & GT & - & $256 \times 192$ & 1.93 & 75.4 \\ 
            % & RTMPose-l & CSPNeXt-l & GT & - & $256 \times 192$ & 4.16 & 76.9 \\ 
            % \cmidrule{2-9}
            & RTMPose-t & CSPNeXt-t & Faster-RCNN  & N/A & $256 \times 192$ & 0.36 & 65.8 &\multirow{4}{*}{-}\\ 
            & RTMPose-s & CSPNeXt-s & Faster-RCNN  & N/A & $256 \times 192$ & 0.68 & 69.6 \\ 
            & RTMPose-m & CSPNeXt-m & Faster-RCNN  & N/A & $256 \times 192$ & 1.93 & 73.6 \\ 
            & RTMPose-l & CSPNeXt-l & Faster-RCNN  & N/A & $256 \times 192$ & 4.16 & 74.8 \\ 
            \cmidrule{2-9}
   %          & RTMPose-tiny* & CSPNeXt-tiny & GT & - & $256 \times 192$ & 0.36 & 67.9 &\multirow{20}{*}{AIC(220K)}\\ 
   %          & RTMPose-s* & CSPNeXt-s & GT & - & $256 \times 192$ & 0.68 & 72.1 \\ 
   %          & RTMPose-m* & CSPNeXt-m & GT & - & $256 \times 192$ & 1.93 & 75.9 \\ 
   %          & RTMPose-l* & CSPNeXt-l & GT & - & $256 \times 192$ & 4.16 & 77.4 \\ 
   %          \cmidrule{2-8}
			% & RTMPose-tiny$^\dag$ & CSPNeXt-tiny & GT & - & $256 \times 192$ & 0.36 & 68.4 & \\ 
   %          & RTMPose-s$^\dag$ & CSPNeXt-s & GT & - & $256 \times 192$ & 0.68 & 72.8 \\ 
   %          & RTMPose-m$^\dag$ & CSPNeXt-m & GT & - & $256 \times 192$ & 1.93 & 77.3 \\ 
   %          & RTMPose-l$^\dag$ & CSPNeXt-l & GT & - & $256 \times 192$ & 4.16 & 78.3 \\ 
   %          \cmidrule{2-8}
            & RTMPose-t & CSPNeXt-t & YOLOv3 & $608 \times 608$ & $256 \times 192$ & 0.36 & 66.0&\multirow{18}{*}{AIC(220K)} \\ 
            & RTMPose-s & CSPNeXt-s & YOLOv3 & $608 \times 608$ & $256 \times 192$ & 0.68 & 70.3 \\ 
            & RTMPose-m & CSPNeXt-m & YOLOv3 & $608 \times 608$ & $256 \times 192$ & 1.93 & 74.7 \\ 
            & RTMPose-l & CSPNeXt-l & YOLOv3 & $608 \times 608$ & $256 \times 192$ & 4.16 & 75.7 \\ 
            \cmidrule{2-8}
            & RTMPose-t & CSPNeXt-t & Faster-RCNN & N/A & $256 \times 192$ & 0.36 & 67.1 \\ 
            & RTMPose-s & CSPNeXt-s & Faster-RCNN & N/A & $256 \times 192$ & 0.68 & 71.1 \\ 
            & RTMPose-m & CSPNeXt-m & Faster-RCNN & N/A & $256 \times 192$ & 1.93 & 75.3 \\ 
            & RTMPose-l & CSPNeXt-l & Faster-RCNN & N/A & $256 \times 192$ & 4.16 & 76.3 \\ 
            \cmidrule{2-8}
            & RTMPose-t & CSPNeXt-t & PicoDet-s & $320 \times 320$ & $256 \times 192$ & 0.36 & 64.3 \\ 
            & RTMPose-s & CSPNeXt-s & PicoDet-s & $320 \times 320$ & $256 \times 192$ & 0.68 & 68.8 \\ 
            & RTMPose-m & CSPNeXt-m & PicoDet-s & $320 \times 320$ & $256 \times 192$ & 1.93 & 73.2 \\ 
            & RTMPose-l & CSPNeXt-l & PicoDet-s & $320 \times 320$ & $256 \times 192$ & 4.16 & 74.2 \\ 
            \cmidrule{2-8}
            & RTMPose-t & CSPNeXt-t & RTMDet-nano & $320 \times 320$ & $256 \times 192$ & 0.36 & 64.4 \\ 
            & RTMPose-s & CSPNeXt-s & RTMDet-nano & $320 \times 320$ & $256 \times 192$ & 0.68 & 68.5 \\ 
            & RTMPose-m & CSPNeXt-m & RTMDet-nano & $320 \times 320$ & $256 \times 192$ & 1.93 & 73.2 \\ 
            & RTMPose-l & CSPNeXt-l & RTMDet-nano & $320 \times 320$ & $256 \times 192$ & 4.16 & 74.2 \\ 
            & RTMPose-m & CSPNeXt-m & RTMDet-m & $640 \times 640$ & $256 \times 192$ & 1.93 & 75.7 \\ 
            & RTMPose-l & CSPNeXt-l & RTMDet-m & $640 \times 640$ & $256 \times 192$ & 4.16 & 76.6 \\ 
			\bottomrule
		\end{tabular}
	}
	\end{center}
\end{table*}
\paragraph{More epochs and multi-dataset training}
When increasing the number of training epochs, the performance of our model can be further improved, reaching 73.5\% AP and 73.7\% AP when training 270 and 420 epochs, respectively.  To obtain higher performance, we combine COCO~\cite{lin2014coco} and AI Challenger~\cite{JiahongWu2017AIC} together for pre-training and fine-tuning. After we sample data from different datasets to form batches according to a balanced sampling ratio, the performance finally achieves 75.3\% AP.

\subsection{Inference pipeline}
To further reduce the overall latency of the top-down algorithm when performing inference, we use the same skip-frame detection mechanism as BlazePose~\cite{blazepose}. Instead of calling the human detector at every frame, we call it every K frames, with K provided as an adjustable hyper-parameter to the user. We maintain a list of bboxes, and when the detector is called we overwrite it with the detection results, and then cropping the input image by the bboxes and scaling them to the specified input size for inference. When all the pose estimation is done, we will post-process the results and generate new bboxes with the external frames of keypoints to update the bbox list. When the human detector is not called, we will directly use the bbox list returned from the previous frame. In addition, we will smooth the result of pose estimation, conduct OKS-based pose NMS, and update the bbox list in the post-processing stage.


==> sections/bak/related_work_bak.tex <==
% !TEX root = ../main.tex
% \setParDis
\section{Related Work}

\begin{figure*}[t]
    \centering
    \includegraphics[width=1\textwidth]{./figs/rtmpose_arch2.pdf}
    % \vspace{-.8em}
    \caption{The overall architecture of RTMPose, which contains a convolutional layer, a fully-connected layer and a Gated Attention Unit(GAU) to refine K keypoint representations. After that 2d pose estimation is regarded as two classification tasks for x-axis and y-axis coordinates to predict the horizontal and vertical location of keypoints.} 
    \label{fig:model}
    % \vspace{-1.5em}
\end{figure*}

\paragraph{Bottom-up Approaches.} 
%
The bottom-up algorithms ~\cite{pishchulin2016deepcut, cao2017realtime, newell2017associative, luo2021rethinking, cheng2020higherhrnet, dekr, kreiss2019pifpaf, jin2020differentiable}, detect all the keypoints of human in an image and combine them to obtain the human pose. However, the accuracy of these algorithms tends to be unstable when the scale of people in the image varies, as some small human components may not be easily detected due to the limitations of feature map resolution. To ensure accuracy, these algorithms often require a larger input resolution, which can lead to a difficult trade-off between speed and accuracy. Although the inference time of bottom-up methods is less affected by the number of humans in the image, this approach still requires relatively high inference times due to the large resolution. For example, OpenPose~\cite{openpose}, an open-source library based on the bottom-up algorithm, can only achieve real-time performance on GPUs and may not be suitable for use on edge devices.

\paragraph{Top-down Approaches.} 
%
The top-down paradigm, also known as a two-stage approach, uses a trained detector to provide bounding boxes and then crops the human to a uniform scale for pose estimation. Algorithms of the top-down paradigm (e.g. SimpleBaseline~\cite{xiao2018simple}, UDP~\cite{huang2020devil}, DARK~\cite{Zhang_2020_CVPR}, ViTPose~\cite{xu2022vitpose}, PSA~\cite{liu2021polarized}, RSN~\cite{cai2020learning}) have been dominating public benchmarks. This approach uses the idea of partitioning to simplify the multi-person pose estimation. The two-stage inference paradigm allows both the human detector and the pose estimator to use relatively small input resolutions, which allows them to outperform bottom-up algorithms in terms of speed and accuracy in non-extreme scenarios (i.e. when the number of people in the image is no more than 6). Additionally, most previous work has focused on achieving state-of-the-art performance on public datasets, while our work aims to design models with better speed-accuracy trade-offs to meet the needs of industrial applications.
%

\paragraph{SimCC.} 
SimCC~\cite{SimCC} is a new method that does not belong to heatmap-based~\cite{xiao2018simple, huang2020devil, Zhang_2020_CVPR, xu2022vitpose} and regression-based methods~\cite{Toshev_2014_CVPR, li2021human, mao2022poseur}, it has a very simple structure, using one $1\times1$ convolution layer to transform the feature dimensions to the number of keypoints. Then features are directly flattened into a sequence $X \in R^{K \times d}$, i.e., \texttt{K} d-dimensional feature vectors where $d = H \times W$. The key idea of SimCC is to regards 2d human pose estimation as two classification tasks for x-axis and y-axis coordinates and to reduce quantization error by dividing each pixel to multiple bins.
In addition to the standard one-hot form, inspired by the label smoothing, SimCC also proposes a Gaussian label smoothing to smooth the training label into a Gaussian distribution. This technique introduces an inductive bias in the soft labels to give higher weights to pixels that are close to GT, thus greatly improving the model performance. We find that this technique is very similar to the idea of the SORD~\cite{sord} algorithm in ordinal regression task. These soft labels naturally encapsulate the rank likelihoods of an input instance given a pre-defined interclass penalty distance $\phi$.

\paragraph{Transformer-based Models.} 
%
Recent advances in natural language processing (NLP) have been made possible by the successful application of the Transformer model, which has also been used in several works (e.g., ViT~\cite{dosovitskiy2020vit}, DETR~\cite{detr}, ViTDet~\cite{vitdet}, ViTPose~\cite{xu2022vitpose}) in the field of computer vision. In particular, studies such as ViTPose~\cite{xu2022vitpose}, TransPose~\cite{yang2021transpose}, TokenPose~\cite{li2021tokenpose}, and Poseur~\cite{mao2022poseur} have shown promising results by incorporating elements of the Transformer model in the task of pose estimation. TokenPose~\cite{li2021tokenpose} and Poseur~\cite{mao2022poseur} adopt ViT's approach of representing keypoints with learnable embedding vectors. TokenPose~\cite{li2021tokenpose} uses a Transformer encoder to process both keypoint tokens and pixel tokens, allowing the model to learn both pixel information and structural information using self-attention. Poseur~\cite{mao2022poseur}, on the other hand, uses a Transformer decoder with a cross-attention mechanism to let the keypoint tokens learn location information and explicitly regress the keypoint coordinates at each layer. TransPose~\cite{yang2021transpose} straightens the 2D feature maps of keypoints extracted by a CNN-based model, uses a Transformer encoder to learn the long-range dependencies between the predicted feature maps on different channels, and then deforms the feature maps back into 2D.
%
Previous works on pose estimation using the Transformer model have either used a heatmap-based representation or retained both pixel tokens and keypoint tokens, which can result in high computation requirements and make real-time inference difficult. In contrast, our approach uses a SimCC-based representation to capture keypoint dependencies using a self-attention mechanism, which significantly reduces the computation load. This allows us to perform real-time inference and achieve better performance in terms of accuracy and efficiency.

